DirectProbe: Studying Representations without Classifiers

Understanding how linguistic structures are encoded in contextualized embedding could help explain their impressive performance across NLP@. Existing approaches for probing them usually call for training classifiers and use the accuracy, mutual information, or complexity as a proxy for the representation's goodness. In this work, we argue that doing so can be unreliable because different representations may need different classifiers. We develop a heuristic, DirectProbe, that directly studies the geometry of a representation by building upon the notion of a version space for a task. Experiments with several linguistic tasks and contextualized embeddings show that, even without training classifiers, DirectProbe can shine light into how an embedding space represents labels, and also anticipate classifier performance for the representation.

==> experiments.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we empirically verify that the clusters we
find in \Cref{sec:dectecting} can reveal different
properties of a given representation.


\subsection{Distances between Clusters}

In this subsection, we analyze the clusters based on the
pair-wise distances. We find that the distances between
clusters are highly correlated with the classification
performance.


% \begin{table}[]
% \begin{tabular}{cccc}
% \toprule
%         & small dis & medium dis & large dis \\ \midrule
% SS-Role & 0.9869    & 0.0131     & 0         \\
% SS-Fun  & 0.9934    & 0.0066     & 0         \\
% SR      & 0.9735    & 0.0250      & 0.0015      \\
% POS     & 0.9979   & 0.0021     & 0         \\
% Dep     & 0.9998    & 0.0002      & 0         \\ \bottomrule
% \end{tabular} \caption{Error distribution with respect to
%     the distance category of pair of labels.}\label{tb:dis-error-rate}
% \end{table}


\subsection{Clusters as Parameters-free Classifier}
In \Cref{sec:by-product}, we discussed about using the
clusters as a parameters-free classifier by assigning the
unlabelled test pint to its closest cluster. We call the
accuracy of this assignment intra-accuracy.



==> fig_decision_boundaries.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \draw [fill] (6,5) circle [radius=0.15];
        \draw [fill] (5.7,4.6) circle [radius=0.15];
        \draw [fill] (5.5,5) circle [radius=0.15];

        \draw [fill] (3,3.5) rectangle (3.3,3.8);
        \draw [fill] (2.5,3) rectangle (2.8,3.3);
        \draw [fill] (3.5,3) rectangle (3.8,3.3);

        \draw [thick] (3.2,5) -- (6.5,2.5);
        \draw [thick] (5.3,5.5) -- (4.2,2.5);

        \draw [thick] (2.5,4.5) .. controls (4.5,4) .. (3.8,2.3);

        \node at (6,4.2) {$B$};
        \node at (3.2,3) {$A$};

        \node at (5.0,5.5) {$h_1$};
        \node at (6.0,2.5) {$h_2$};
        \node at (2.3,4.3) {$h_3$};
    \end{tikzpicture}
    \caption{A set of hypothesis functionss provided by the
    representation. $h_1,h_2$ and $h_3$ are all valid
    hypothesis for this simple binary
    classification problem. The signal expressed by the
    representation is the set of all hypothesis
    that can fit the data.}\label{fig:decision-boundaries}
\end{figure}


==> heuristic.tex <==
\section{Heuristic Algorithm}\label{sec:heuristic}


==> notes.tex <==
\begin{itemize}
    \item Because of the limited space, I give up the point
        that the best classifier is not necessarily a linear
        one even if the space is linear separable
    \item Add labels to the appendix. Fix the all refs in
        the main text.
    \item Connection to the information theory.
\end{itemize}


==> quality2.tex <==
\section{Representations and Learning}\label{sec:quality}
In this section, we first briefly review the relationship
between representations and model learning. Then, we propose
the definition of the signals expressed by the
representation.

\subsection{Two Sub-tasks of A Learning
Problem}\label{sec:subtasks}

A learning problem usually can be divided into two
sub-problems: representing data and learning a
model~\cite{bengio2013representation}. The former involves
transforming input objects $x$, \eg words, pairs of words or
sentences, into a representation $E(x)\in\mathcal{R}^n$ that
provides the features for the latter.  Model learning builds
a classifier $h$ by learning the signals expressed by the
representation to make a prediction, denoted by the composed
function $h(E(x))$. 

\Cref{fig:subworks} illustrates the two sub-tasks, and their
role in figuratively ``transporting'' inputs $x$ to outputs
with the probability of error less than some small
$\epsilon$. However, representations $E_i$ are evaluated
jointly by the composition of the representations $E_i$ with
the classifiers
$h_i$~\cite{peters-etal-2019-tune,tenney2018what,conneau-etal-2018-cram}.
Thus, the perceived quality of a representation is affected
by many factors involving the classifiers, \eg~starting
points, or optimization algorithms. A bad predictive
performance does not necessarily mean a bad representation
and vice versa.  In our supersense prediction task, the
accuracy of different runs of the same classifier and
representation can be as large as $9.63\%$, which cannot be
ignored.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{../resources/subworks.pdf}
    \caption{The total work in the learning problem is
    visualized as the distance traveled from the input bar
    to the output bar. Different representations $E_i$ and
    different classifiers $h_i$ provides different effort.
    }\label{fig:subworks}
\end{figure}

The problem can be alleviated by restricting the classifier
to be linear for all representations and comparing the final
performance~\cite{alain2016understanding,liu-etal-2019-linguistic,hewitt-manning-2019-structural}.
However, this simple solution is not ideal. A linear model
need not be the best classifier on top of the singals
expressed by the representation. Ideally, the solution is we
choose the highest-performing classifier aomong all the
possible classifiers as the
probe~\cite{pimentel-etal-2020-information}. However,
enumerating all the possible classifiers is computationally
intracable.

\subsection{Signals of Representations}\label{sec:signal}
We propose to disentangle the evaluation of a representation
$E_i(x)$ from the classifiers that are trained over it and
analyze the signals expressed by the representation directly.
To do so, the first step is to define the signals expressed
by a representation.

Classifiers are trained to find a simple (according to
Occam's Rzaor) hypothesis $h^{*}$ that can achieve low
training error and then evaluated on a test set. That
hypothesis $h^{*}$ is decided by:
\begin{inparaenum}[(i)]
    \item the model family $H$ (\eg a linear model or a two
        layers neural network);
    \item the representation space $E$ on the training set.
\end{inparaenum}

The representation space $E$ provides a set of hypothesis
and the learning model choose one of them.  This process is
illustrated by \Cref{fig:decision-boundaries}. There are two
linear hypothesis ($h_1$ and $h_2$) and one non-linear
hypothesis ($h_3$). They are all valid for this
binary classification problem. A learning process can return
any one of them.  Inspired by this, we define the
signal expressed by a representation as the set of
hypothesis such that:
\begin{inparaenum}[(i)]
    \item \textit{achieve the training error less than
    $\epsilon$};
    \item \textit{with at most $\eta$ complexity.}
\end{inparaenum}

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{../resources/decision-boundaries.pdf}
    \caption{A set of hypothesis functionss provided by the
    representation. $h_1,h_2$ and $h_3$ are all valid
    hypothesis for this simple binary
    classification problem. The signal expressed by the
    representation is the set of all hypothesis
    that can fit the data.}\label{fig:decision-boundaries}
\end{figure}

Let us formalize this definition. Suppose $\mathcal{H}$
represents the whole hypothesis space, consisting of all
possible classifiers of interest (lower-cased $h$). Let
$C(E, h)$ denote the complexity of the hypothesis $h$ for
the representation $E$. For example, the complexity could be
defined by the number of parameters in the model, their
$VC$-dimension, or other formal properties of the hypothesis
$h$.

We can now define the signals $V(E,D)$ expressed by a representation
$E$ on a task $D$ as:

\begin{equation}
    \small
    V(E,D) \triangleq \{h\vert Error_T(h,E,D)\le\epsilon,
    C(E,h)\le\eta, h\in\mathcal{H}\}.
    \label{eq:def}
\end{equation}

where $Error_{T}$ represents the training error.


Different properties of the hypothesis $h\in V_(E,D)$ are
used as a measurement of the representation $E$. Common
usage includes generalization
error~\cite{goodwin-etal-2020-probing,kim-etal-2019-probing,yaghoobzadeh-etal-2019-probing},
mutual
information~\cite{pimentel-etal-2020-information,voita2020information}
and complexity~\cite{pimentel2020pareto}.  Following the
most commonly usage, in this work, we also use the
generalization error as a measurment of representation $E$.

As we mentioned in \cref{sec:subtasks}, it is impossible to
find $V(E,D)$ by enumerating $\mathcal{H}$. Previous work
approximated $V(E,D)$ by restricting $C(E,h)$ to be equal to
a certain $\eta$ (\eg, fixing the probe to be a linear
model) and $\mathcal{H}$ to be a finite (small set?) set.
We argue that kind of approximation is incomplete.  Instead,
we propose to directly detect $V(E,D)$ without imposing any
restrictions. 



==> verification.tex <==
\section{Verification}\label{sec:verification}

\subsection{Complexity of Representation}

More clusters means more piece-wise linear functions; more
linear functions means more complicated the decision
boundary.

\subsection{Predication of Generalization Error}
\begin{itemize}
    \item Two ways of predication: with or without a test
        set.
    \item Minimum distances between convex hulls can be the
        indicator of generalization error.
    \item Formualization of finding such distances.

    \item Loose lower bound and upper bound of
        classification performance on a given test set.
    \item Formualization of finding the minimum distance
        between test points and convex hulls.
\end{itemize}


